Lightweight Channel-wise Dynamic Fusion Model: Non-stationary Time Series Forecasting via Entropy Analysis

Non-stationarity is an intrinsic property of real-world time series and plays a crucial role in time series forecasting. Previous studies primarily adopt instance normalization to attenuate the non-stationarity of original series for better predictability. However, instance normalization that directly removes the inherent non-stationarity can lead to three issues: (1) disrupting global temporal dependencies, (2) ignoring channel-specific differences, and (3) producing over-smoothed predictions. To address these issues, we theoretically demonstrate that variance can be a valid and interpretable proxy for quantifying non-stationarity of time series. Based on the analysis, we propose a novel lightweight \textit{C}hannel-wise \textit{D}ynamic \textit{F}usion \textit{M}odel (\textit{CDFM}), which selectively and dynamically recovers intrinsic non-stationarity of the original series, while keeping the predictability of normalized series. First, we design a Dual-Predictor Module, which involves two branches: a Time Stationary Predictor for capturing stable patterns and a Time Non-stationary Predictor for modeling global dynamics patterns. Second, we propose a Fusion Weight Learner to dynamically characterize the intrinsic non-stationary information across different samples based on variance. Finally, we introduce a Channel Selector to selectively recover non-stationary information from specific channels by evaluating their non-stationarity, similarity, and distribution consistency, enabling the model to capture relevant dynamic features and avoid overfitting. Comprehensive experiments on seven time series datasets demonstrate the superiority and generalization capabilities of CDFM.

==> table/ablation.tex <==
\begin{table*}[t]
\caption{Ablation study of CDFM components. ‘\(\alpha=1\)’ refers to including all channels in the fusion process. 'Static Weight' refers to a model that employs a trainable static matrix, shared across all samples, as the fusion weights.}
\centering
\footnotesize
\large
%\setlength{\tabcolsep}{1.mm}

\renewcommand{\arraystretch}{0.95}
\resizebox{0.96\textwidth}{!}{
\begin{tabular}{c|c|c|c|c|cccc|cccc}
\toprule
\multicolumn{2}{c|}{Dual-predictor}                                                                                                              &                                    &                                                                                      &                          & \multicolumn{4}{c|}{ETTh1}                                                                                                                                     & \multicolumn{4}{c}{ETTh2}                                                                                                                                     \\ \cmidrule(rl){1-2} \cmidrule(rl){6-13}
\begin{tabular}[c]{@{}c@{}}Time Stationary \\ Predictor\end{tabular} & \begin{tabular}[c]{@{}c@{}}Time Non-stationary \\ Predictor\end{tabular} & \multirow{-2}{*}{\begin{tabular}[c]{@{}c@{}}Channel \\ Selector\end{tabular}} & \multirow{-2}{*}{\begin{tabular}[c]{@{}c@{}}Dynamic Weight \\ Learner\end{tabular}} & \multirow{-2}{*}{Metric} & 96                                    & 192                                   & 336                                   & 720                                   & 96                                    & 192                                   & 336                                   & 720                                   \\ \midrule
                                                                     &                                                                          &                                    &                                                                                      & MSE                      & 0.384                                 & 0.436                                 & 0.479                                 & 0.481                                 & 0.289                                 & 0.375                                 & 0.417                                 & 0.42                                  \\
\multirow{-2}{*}{\checkmark}                                                  & \multirow{-2}{*}{}                                                       & \multirow{-2}{*}{}                 & \multirow{-2}{*}{}                                                                   & MAE                      & 0.392                                 & 0.422                                 & 0.445                                 & 0.469                                 & 0.337                                 & 0.389                                 & 0.426                                 & 0.439                                 \\ \midrule
                                                                     &                                                                          &                                    &                                                                                      & MSE                      & 0.398                                 & 0.434                                 & 0.499                                 & 0.508                                 & 0.315                                 & 0.432                                 & 0.486                                 & 0.732                                 \\
\multirow{-2}{*}{}                                                   & \multirow{-2}{*}{\checkmark}                                                      & \multirow{-2}{*}{}                 & \multirow{-2}{*}{}                                                                   & MAE                      & 0.410                                 & 0.427                                 & 0.477                                 & 0.503                                 & 0.374                                 & 0.447                                 & 0.481                                 & 0.614                                 \\ \midrule
                                                                     &                                                                          &                                    &                                                                                      & MSE                      & 0.379                                 & 0.428                                 & 0.467                                 & 0.461                                 & 0.286                                 & 0.369                                 & 0.402                                 & 0.392                                 \\
\multirow{-2}{*}{\checkmark}                                                  & \multirow{-2}{*}{\checkmark}                                                      & \multirow{-2}{*}{\checkmark}                & \multirow{-2}{*}{Static Weight}                                                      & MAE                      & 0.391                                 & 0.420                                  & 0.440                                  & 0.457                                 & 0.336                                 & 0.387                                 & 0.415                                 & 0.418                                 \\ \midrule
                                                                     &                                                                          &                                    &                                                                                      & MSE                      & 0.379                                 & 0.429                                 & 0.478                                 & 0.479                                 & 0.322                                 & 0.381                                 & 0.429                                 & 0.489                                 \\
\multirow{-2}{*}{\checkmark}                                                  & \multirow{-2}{*}{\checkmark}                                                      & \multirow{-2}{*}{\(\alpha=1\)}          & \multirow{-2}{*}{\checkmark}                                                                  & MAE                      & 0.392                                 & 0.421                                 & 0.445                                 & 0.468                                 & 0.365                                 & 0.406                                 & 0.446                                 & 0.491                                 \\ \midrule
                                                                     &                                                                          &                                    &                                                                                      & MSE                      & {\color[HTML]{FF0000} \textbf{0.373}} & {\color[HTML]{FF0000} \textbf{0.426}} & {\color[HTML]{FF0000} \textbf{0.465}} & {\color[HTML]{FF0000} \textbf{0.458}} & {\color[HTML]{FF0000} \textbf{0.283}} & {\color[HTML]{FF0000} \textbf{0.366}} & {\color[HTML]{FF0000} \textbf{0.399}} & {\color[HTML]{FF0000} \textbf{0.388}} \\
\multirow{-2}{*}{\checkmark}                                                  & \multirow{-2}{*}{\checkmark}                                                      & \multirow{-2}{*}{\checkmark}                & \multirow{-2}{*}{\checkmark}                                                                  & MAE                      & {\color[HTML]{FF0000} \textbf{0.389}} & {\color[HTML]{FF0000} \textbf{0.418}} & {\color[HTML]{FF0000} \textbf{0.438}} & {\color[HTML]{FF0000} \textbf{0.454}} & {\color[HTML]{FF0000} \textbf{0.334}} & {\color[HTML]{FF0000} \textbf{0.384}} & {\color[HTML]{FF0000} \textbf{0.413}} & {\color[HTML]{FF0000} \textbf{0.415}} \\ \bottomrule
\end{tabular}}

\label{tab: tab6}
\end{table*}

==> table/ablation_channel.tex <==
\begin{table*}[h]
\caption{Detailed ablation results on Channel Selector.}
\centering
\footnotesize
\large
%\setlength{\tabcolsep}{1.mm}

\renewcommand{\arraystretch}{0.80}
\resizebox{0.76\textwidth}{!}{
\begin{tabular}{c|c|cc|cc|cc|cc}
\toprule
\multicolumn{2}{c|}{Models}    & \multicolumn{2}{c|}{CDFM}                                                      & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}w/o Non- \\ stationarity\end{tabular}} & \multicolumn{2}{c|}{w/o Similarity} & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}w/o Distribution \\ Consistency\end{tabular}  } \\ \midrule
\multicolumn{2}{c}{Metric}    & MSE                                   & MAE                                   & MSE                 & MAE                & MSE              & MAE             & MSE                     & MAE                    \\ \midrule
                        & 96  & {\color[HTML]{FF0000} \textbf{0.374}} & {\color[HTML]{FF0000} \textbf{0.389}} & 0.385               & 0.393              & 0.374            & 0.389           & 0.374                   & 0.389                  \\
                        & 192 & {\color[HTML]{FF0000} \textbf{0.426}} & {\color[HTML]{FF0000} \textbf{0.419}} & 0.436               & 0.422              & 0.426            & 0.419           & 0.426                   & 0.419                  \\
                        & 336 & {\color[HTML]{FF0000} \textbf{0.465}} & {\color[HTML]{FF0000} \textbf{0.438}} & 0.479               & 0.445              & 0.465            & 0.438           & 0.465                   & 0.438                  \\
\multirow{-4}{*}{ETTh1} & 720 & {\color[HTML]{FF0000} \textbf{0.459}} & {\color[HTML]{FF0000} \textbf{0.455}} & 0.490               & 0.476              & 0.459            & 0.455           & 0.459                   & 0.455                  \\  \midrule
                        & 96  & {\color[HTML]{FF0000} \textbf{0.285}} & {\color[HTML]{FF0000} \textbf{0.335}} & 0.285               & 0.335              & 0.286            & 0.336           & 0.350                   & 0.393                  \\
                        & 192 & {\color[HTML]{FF0000} \textbf{0.366}} & {\color[HTML]{FF0000} \textbf{0.385}} & 0.366               & 0.385              & 0.367            & 0.386           & 0.385                   & 0.395                  \\
                        & 336 & {\color[HTML]{FF0000} \textbf{0.400}} & {\color[HTML]{FF0000} \textbf{0.414}} & 0.400               & 0.414              & 0.403            & 0.417           & 0.472                   & 0.481                  \\
\multirow{-4}{*}{ETTh2} & 720 & {\color[HTML]{FF0000} \textbf{0.389}} & {\color[HTML]{FF0000} \textbf{0.416}} & 0.389               & 0.416              & 0.436            & 0.453           & 0.455                   & 0.454                 
 \\ \bottomrule
\end{tabular}}

\label{tab: tab6}
\end{table*}

==> table/efficiency.tex <==
\begin{table*}[t]
\caption{Static and runtime metrics of CDFM and other mainstream models on the ETTm1 and Weather Dataset with a forecast horizon of 720.}
\centering
\small
\setlength{\tabcolsep}{1.7mm}
\begin{tabular}{c|ccc|ccc}
\toprule
Dataset         & \multicolumn{3}{c|}{ETTm1}                                                                                                                                          & \multicolumn{3}{c}{Weather}                                                                                                                                        \\ \midrule
Metric        & MSE                                   & {\begin{tabular}[c]{@{}c@{}}Training Time \\ (ms/iter)\end{tabular}}  & {\begin{tabular}[c]{@{}c@{}}Memory \\ (MB)\end{tabular}}  & MSE                                   & {\begin{tabular}[c]{@{}c@{}}Training Time \\ (ms/iter)\end{tabular}} & {\begin{tabular}[c]{@{}c@{}}Memory \\ (MB)\end{tabular}}  \\ \midrule
iTransformer  & 0.487                                 & 30.45                                                            & 0.29                                                 & 0.358                                 & 59.16                                                             & 4.92                                                 \\
TimeMixer     & {\textcolor{blue} {\ul 0.462}} & 91.72                                                             & {\textcolor{blue} {\ul 0.26}}                    & 0.345                                 & 118.59                                                             & 0.29                                                 \\
PatchTST      & 0.466                                 & 53.86                                                             & 1.44                                                 & 0.351                                 & 60.35                                                             & 1.44                                                 \\
TimesNet      & 0.484                                 & 125.43                                                             & 0.71                                                 & 0.355                                 & 264.30                                                            & 1.35                                                 \\
DLinear       & 0.478                                 & {\color[HTML]{FF0000} \textbf{11.94}}                              & {\color[HTML]{FF0000} \textbf{0.13}}                 & 0.347                                 & {\textcolor{blue} {\ul 13.87}}                                 & {\color[HTML]{FF0000} \textbf{0.13}}              \\ \midrule
\textbf{CDFM (Ours)} & \color[HTML]{FF0000} \textbf{0.456}    & {\textcolor{blue} {\ul 20.57}}                                & 0.27                                                 & {\color[HTML]{FF0000} \textbf{0.322}} & {\color[HTML]{FF0000} \textbf{12.49}}                              & {\textcolor{blue} {\ul 0.27}}         \\ \bottomrule          
\end{tabular}

\label{tab: tab8}
\end{table*}

==> table/nonstationary_short_short.tex <==
\begin{table}[t]
\caption{Comparison between CDFM and non-stationary approaches with different prediction lengths \(H \in
\{96, 192, 336, 720\}\) and the input length \(L = 96\). Best results are highlighted in {\color[HTML]{FF0000} \textbf{red}} and the second {\textcolor{blue} {\ul underlined}}.}
\centering
\large
%\setlength{\tabcolsep}{1.5mm}
\renewcommand{\arraystretch}{1.0}
\resizebox{0.45\textwidth}{!}{
\begin{tabular}{c|cc|cc|cc}
\toprule
Dataset         & \multicolumn{2}{c|}{ETTh1}                                                     & \multicolumn{2}{c|}{ETTm1}                                                     & \multicolumn{2}{c}{Weather}                                                   \\ \midrule
Metric          & MSE                                   & MAE                                   & MSE                                   & MAE                                   & MSE                                   & MAE                                   \\ \midrule
NS-Trans(2022)  & 0.679                                 & 0.563                                 & 0.524                                 & 0.468                                 & 0.282                                 & 0.307                                 \\
Koopa(2023)     & 0.454                                 & 0.443                                 & 0.399                                 & {\textcolor{blue} {\ul 0.406}}    & 0.245                                 & {\textcolor{blue} {\ul 0.272}}    \\
HTV-Trans(2024) & 0.457                                 & {\textcolor{blue} {\ul 0.440}}    & 0.406                                 & 0.406                                 & 0.258                                 & 0.284                                 \\
TFPS(2024)      & {\textcolor{blue} {\ul 0.448}}    & 0.443                                 & {\textcolor{blue} {\ul 0.395}}    & 0.407                                 & {\color[HTML]{FF0000} \textbf{0.241}} & {\color[HTML]{FF0000} \textbf{0.271}} \\ \midrule
CDFM(ours)      & {\color[HTML]{FF0000} \textbf{0.431}} & {\color[HTML]{FF0000} \textbf{0.425}} & {\color[HTML]{FF0000} \textbf{0.386}} & {\color[HTML]{FF0000} \textbf{0.393}} & {\textcolor{blue} {\ul 0.243}}    & 0.285                                \\ \bottomrule
\end{tabular}}


\label{tab: tab4}
\end{table}

==> table/results_short.tex <==

\begin{table*}[t]
\caption{Multivariate forecasting results on all seven datasets with different prediction lengths \(H \in
\{96, 192, 336, 720\}\) and the input length \(L=96\).  Best results are highlighted in {\color[HTML]{FF0000} \textbf{red}} and the second {\textcolor{blue} {\ul underlined}}. Full results and more comparison results on \textit{searched hyperparameter} input lengths are available in Appendix~\ref{sec: full results}.}
\centering
\large
%\setlength{\tabcolsep}{1.5mm}
\renewcommand{\arraystretch}{0.85}
\resizebox{0.98\textwidth}{!}{
\begin{tabular}{c|cc|cc|cc|cc|cc|cc|cc}
\toprule
Dataset            & \multicolumn{2}{c|}{ETTh1}                                                     & \multicolumn{2}{c|}{ETTh2}                                                     & \multicolumn{2}{c|}{ETTm1}                                                     & \multicolumn{2}{c|}{ETTm2}                                                     & \multicolumn{2}{c|}{Weather}                                                   & \multicolumn{2}{c|}{Exchange\_rate}                                            & \multicolumn{2}{c}{Electricity}                                               \\ \midrule
Metric             & MSE                                   & MAE                                   & MSE                                   & MAE                                   & MSE                                   & MAE                                   & MSE                                   & MAE                                   & MSE                                   & MAE                                   & MSE                                   & MAE                                   & MSE                                   & MAE                                   \\ \midrule
repeat             & 1.321                                 & 0.737                                 & 0.539                                 & 0.481                                 & 1.271                                 & 0.698                                 & 0.385                                 & 0.394                                 & 0.352                                 & 0.320                                 & {\textcolor{blue} {\ul 0.341}}    & {\textcolor{blue} {\ul 0.390}}    & 1.612                                 & 0.958                                 \\
FEDformer(2022)    & 0.455                                 & 0.465                                 & 0.439                                 & 0.449                                 & 0.424                                 & 0.443                                 & 0.301                                 & 0.350                                 & 0.319                                 & 0.372                                 & 0.512                                 & 0.495                                 & 0.210                                 & 0.323                                 \\
DLinear(2023)      & 0.460                                 & 0.454                                 & 0.491                                 & 0.479                                 & 0.405                                 & 0.409                                 & 0.308                                 & 0.363                                 & 0.266                                 & 0.316                                 & 0.355                                 & 0.413                                 & 0.210                                 & 0.296                                 \\
TimesNet(2023a)    & 0.458                                 & 0.453                                 & 0.395                                 & 0.416                                 & 0.412                                 & 0.418                                 & 0.291                                 & 0.330                                 & 0.258                                 & 0.286                                 & 0.397                                 & 0.433                                 & 0.194                                 & 0.295                                 \\
PatchTST(2023)     & 0.468                                 & 0.453                                 & 0.384                                 & 0.406                                 & 0.393                                 & 0.406                                 &{\textcolor{blue} {\ul 0.284}}                                 & {\textcolor{blue} {\ul 0.327}}                                 & 0.258                                 & 0.280                                 & 0.358                                 & 0.402                                 & 0.190                                 & 0.276                                 \\
FITS(2024)         & 0.456                                 & 0.446                                 & {\textcolor{blue} {\ul 0.378}}    & {\textcolor{blue} {\ul 0.401}}    & 0.414                                 & 0.408                                 & 0.286                                 & 0.329                                 & 0.250                                 & {\textcolor{blue} {\ul 0.279}}    & 0.360                                 & 0.406                                 & 0.218                                 & 0.296                                 \\
TimeMixer(2024)    & {\textcolor{blue} {\ul 0.448}}    & {\textcolor{blue} {\ul 0.439}}    & 0.384                                 & 0.409                                 & {\textcolor{blue} {\ul 0.391}}    & {\textcolor{blue} {\ul 0.400}}    & {\color[HTML]{FF0000} \textbf{0.279}} & {\color[HTML]{FF0000} \textbf{0.324}} & {\textcolor{blue} {\ul 0.245}}    & {\color[HTML]{FF0000} \textbf{0.275}} & 0.417                                 & 0.424                                 & {\textcolor{blue} {\ul 0.183}}    & {\textcolor{blue} {\ul 0.274}}    \\
iTransformer(2024) & 0.457                                 & 0.450                                 & 0.384                                 & 0.407                                 & 0.408                                 & 0.412                                 & 0.293                                 & 0.336                                 & 0.260                                 & 0.281                                 & 0.365                                 & 0.407                                 & {\color[HTML]{FF0000} \textbf{0.182}} & {\color[HTML]{FF0000} \textbf{0.272}} \\ \midrule
CDFM(ours)         & {\color[HTML]{FF0000} \textbf{0.431}} & {\color[HTML]{FF0000} \textbf{0.425}} & {\color[HTML]{FF0000} \textbf{0.360}} & {\color[HTML]{FF0000} \textbf{0.388}} & {\color[HTML]{FF0000} \textbf{0.386}} & {\color[HTML]{FF0000} \textbf{0.393}} & {\textcolor{blue} {\ul 0.284}}    & {\textcolor{blue} {\ul 0.327}}    & {\color[HTML]{FF0000} \textbf{0.241}} & 0.283                                 & {\color[HTML]{FF0000} \textbf{0.289}} & {\color[HTML]{FF0000} \textbf{0.371}} & 0.207                                 & 0.293                                \\ \bottomrule   
\end{tabular}}
\label{tab: tab2}
\end{table*}



